Somesite I Used To Crawl: Awareness, Agency and Efficacy in Protecting Content Creators From AI Crawlers

The success of generative AI relies heavily on training on data scraped through extensive crawling of the Internet, a practice that has raised significant copyright, privacy, and ethical concerns. While few measures are designed to resist a resource-rich adversary determined to scrape a site, crawlers can be impacted by a range of existing tools such as robots.txt, NoAI meta tags, and active crawler blocking by reverse proxies. In this work, we seek to understand the ability and efficacy of today's networking tools to protect content creators against AI-related crawling. For targeted populations like human artists, do they have the technical knowledge and agency to utilize crawler-blocking tools such as robots.txt, and can such tools be effective? Using large scale measurements and a targeted user study of 203 professional artists, we find strong demand for tools like robots.txt, but significantly constrained by critical hurdles in technical awareness, agency in deploying them, and limited efficacy against unresponsive crawlers. We further test and evaluate network-level crawler blockers provided by reverse proxies. Despite relatively limited deployment today, they offer stronger protections against AI crawlers, but still come with their own set of limitations.

==> blocking_old.tex <==
\section{Blocking AI Bots}
% Blocking Practices / Robots.txt enforcement in practice
\alex{
    Alternative structure:
    * Methodology 
        * Inferring for reverse-proxy
        * Inferring for other websites (i.e., anything not Cloudflare and Amazon)
    * Results
    Current 6.4 and 6.5 read like discussion. (or a separate section)
}


High Level: 
At the end of the day, respecting the directives in robots.txt is completely voluntary and relies on the goodwill of the scrapers.
% some challenges with robots.txt
The most famous example is the Perplexity AI case, where the operators were found to be scraping websites that explicitly disallowed them in robots.txt. Furthermore, many AI scrapers, such as anthropic-ai are currently undocumented \todo{check if this is still true}, making it difficult for website operators to add them to robots.txt.
In our previous analysis on GPT Apps, we alsofind that many AI-related fetchers indeed do not respect robots.txt. 
Thus, the natural next step for a website operator who wants to block AI bots from scraping their content is to take \textit{active} blocking measures. 
In this section, we aim to evaluate the practical options availible to website operators for blocking AI bots, measure websites' blocking behavior in practice, and compare it to their stated intent in robots.txt.

Summary
\begin{enumerate}
    \item We evaluate the active blocking measures specifically for AI-related bots that are availible to website operators. Specifically we test 2 major reverse proxies, Cloudflare and Amazon Cloudfront.
    \item We measure the blocking behavior for AI-related bots in practice for the top 10k domains. We compare this behavior to the directives stated in robots.txt.
\end{enumerate}


\subsection{Evaluation of Active Blocking Measures for AI-related Bots} 
In this section, we evaluate the operation of the active blocking measures availible to website operators for blocking AI bots. We focus on two major reverse proxies, Cloudflare and Amazon Cloudfront. Reverse proxies are well-positioned to implement such blocking measures, and together, 32\% of the top 10k sites user either platform. 

\subsubsection{Cloudflare}
Cloudflare recently launched a new option that allows users to "Block AI Crawlers and Scrapers" with the click of a button \cite{cloudflareAIblocking} (Figure \ref{fig:cloudflare_block_ai_crawlers}). We test the operation of this feature and discuss its efficacy. Cloudflare as it has the greatest market share of all reverse proxies \cite{reverseproxymarketshare} and we emperically find that 16\% of the top 10k websites use Cloudflare through inspecting their DNS records. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{plot/cloudflare_bot.png}
    % this image is publicly availible.
    \caption{Cloudflare "Block AI Scrapers and Crawlers" option}
    \label{fig:cloudflare_block_ai_crawlers}
\end{figure}

% Setting inference methodology
\paragraph{Methodology} Cloudflare does not document the list of bots blocked by each setting, nor documents the setting's method of operation, so we must infer both aspects through experimentation. Thus, we sign up for a Cloudflare "free" and "Pro" account. Then, we set up the reverse proxy as per the instructions provided by Cloudflare on two sites we control. 

Using a list of user-agent strings from over 500 different scrapers and crawlers \cite{crawleruseragents}, plus the list of AI-related user-agents from Dark Visitors \cite{darkvisitorsagents}, we visit each website using Cloudflare with each user-agent string. We are able to detect the outcome of each visit by checking the HTTP status code of the response, and detecting whether the response is a Cloudflare Block or Challenge page. We were also able to use the Cloudflare Dashboard and our server's HTTP logs as a source of ground truth.

% Experiement results on our own website
\paragraph{Default blocking configurations} With no blocking options turned on, 5 user-agents are blocked: \textsc{['Python-urllib', 'Nutch', 'Teoma', 'grub.org', 'binlar']}. In the free tier, enabling "Bot Fight Mode" does not seem to block any additional user-agents. \alex{too much detail, likely will move to appendix or cut. Anything not AI doesnt have to be listed.}

The Pro tier allows for slightly more fine-grained configuration of its equivalent "Super Bot Fight Mode": there are 3 options for configuration: Block AI Bots (on/off), "Definately Automated" (which are requests from bots Cloudflare deems as "bad") (Block/Allow/Managed Challenge), and "Verified Bots" (Block/Allow/Managed Challenge). We discovered that the latter 2 options essentially verifies the origin of a given bot request by checking the IP address against the IP address associated the verified bot\footnote{In order to add a verified bot, you must register the bot with Cloudflare. In the registration process, you must provide the bot's user-agent, purpose, and a list of IP addresses requests from the bot will originate from. Cloudflare maintains a list of verified bots, which is publicly availible \cite{cloudflareverifiedbots}.}. If a request claims to be from a verified bot (i.e., its user-agent is one of a verified bot), but its IP address does not match Cloudflare's internal list for that bot, then the requets will be blocked or challenged under the "Definately Automated" rule. Note that since we cannot spoof IP addresses of verified bots, we cannot test the "Verified Bots" rule directly.

\paragraph{Block AI Bots} We find that 15 additional user-agents are blocked when the "Block AI Crawlers" option is enabled: \textsc{'CCBot', 'PiplBot', 'omgili', 'magpie-crawler', 'MeltwaterNews', 'Diffbot/', 'Bytespider', 'Amazonbot', 'AwarioSmartBot', 'AwarioRssBot', 'GPTBot', 'ChatGPT-User', 'YouBot', 'PerplexityBot/', '[cC]laude[bB]ot'}. The behavior of this option is identical for the Free and Pro tiers. Furthermore, we find that Cloudflare "Block AI Crawlers and Scrapers" uses pattern matching on the user-agent string to block AI bots. That is, we find that "GPTBot/*" is blocked by Cloudflare, by "GPTBot" is not. This example demonstrates the fragility of pattern matching based blocking mechanisms as changing the user-agent string even slightly can evade detection.

\paragraph{Definately Automated} This Pro-tier only rule targets "fake" verifed bots\footnote{Note that although we cannot test whether or not the "real" verified bot will be blocked under this setting, it is highly unlikely as Cloudflare deems all verified bots to be "good" bots.}, i.e., bots that claim to be one entity (via the user-agent), but originate from an undocumented IP address. The website operator is able to set this rule to "Allow", "Block", and "Managed Challenged". With the latter option, the visitor is shown a captcha-like screen. We find that 17 of the 500+ bot user agents we tested are blocked by this option as they are verified bots. In addition, 33 non-verfied bots are blocked by this option \todo{this number needs to be updated, i think} \todo{reference to table}. These user-agents are mainly of bots that are known automation tools (e.g., PhantomJS, HeadlessChrome, libwww-perl), but interestingly, include some AI-related bots, such as CCBot, ClaudeBot, PerplexityBot, Bytespider, and anthropic-ai. This means that Cloudflare deems such AI bots to be "bad" bots.
% All the block AI bots setting does in addition to the definately automated setting, is that it block verified AI bots, which include: GPTBot, ChatGPT-User, GoogleOther, Applebot

% i finally realized the point of the Block AI bots setting, given that it is a subset of the block definately automated setting. So customers of cloudflare want to do bot mitigation, right? and there is this notion of "good" and "bad" bots. The standard customer, who dgaf about AI bots, just wants to block "bad" or misbehaved/malicious bots. However, many AI bots, such as GPTBot are well-behaved (i.e., respect robots.txt, don't make too many requests), so they are deemed, from the perspective of the user who does not care about GenAI, as a good bot. However, from the perspective of the user who does care about GenAI, they are unwanted. So the Block AI bots setting is for the latter user, who wants to block "bad" bots, but also wants to block AI bots.

\subsubsection{Amazon Cloudfront}
We evaluate Amazon Cloudfront in a similar manner, through implementing the service on a website we control. We are thus able to use the Cloudfront Bot Management Dashboard and our server logs as ground truth. With respect to block AI-related bots, Cloudfront offers an "Artificial Intellence" category in their bot management product.  
\paragraph{User agents blocked} We tested which user-agents this AI category encompasses. We not that for the AI category, Cloudfront specifically says that it will block regardless of verification status. We find that the Cloudfront AI bots category only blocks GPTBot and GPTUser. 
% Unfortunately, this makes it difficult for us to infer whether or not a site hosted by Cloudfront has this option enable

\subsection{Inferring AI bot blocking of websites in practice}
% how did we test the blocking behavior in practice?
To measure the blocking behavior of websites in practice, we visited the website using a headless browser with a variety of different user agents. Specifically, we first visit with two "regular" user agents, one for the most popular version of Chrome and one for the most popular version of Firefox. We then visit the website with a variety of AI bot user agents, \todo{edit the full list once we have it} including GPTBot, ChatGPT-User, etc. We then record the response of the website for each user-agent string, specifically whether the website returns a 403 Forbidden status code or a 200 OK status code.
\todo{compare content size of the response as well?}

% results
\paragraph{Automation tools can be inherently blocked} We find that 75\% of websites return a 200 OK when we visit with a normal (human) user-agent. We find that 15\% of websites return a 403 Forbidden status code even when we visit with a normal user-agent. This shows that the automation tool we are using to visit the site is inherently blocked. While many advanced bot detection methods exist (e.g., through fingerprinting or behaviorial analysis), we consider this out of scope for our study, which focuses on the most basic case: user-agent based blocking. Thus, we exclude this subset of websites in the proceeding analysis.

\paragraph{Verified bots} Since we can only spoof the user agent and not the IP of a given bot, we cannot pretend to be a "Verified" bot. This means that for sites that do indeed block fake verified bots, we are unable to determine whether the site is blocking us solely because of the user agent or the user agent and IP address combination. 
We thus use fake Googlebot being blocked as a proxy for whether or not a site has implemented these kinds of rules. Furthermore, for some AI-related user agents, their IP address is not documented so any blocking must be implemented on the user-agent level. 
For the subset of sites using Cloudflare, we are also able to infer whether they have have turned on the "Block AI Bots" rule. 

\subsubsection{Inferring Cloudflare AI-blocking settings}
\paragraph{Inferring Cloudflare Settings (Methodology)}
\elisa{I think a lot of this methodology can be moved to the appendix}
Given our findings from testing on our own site, we are able to infer whether a given site using Cloudflare has opted to block AI Crawlers and Scrapers. First, the block "definately automated" option can be used in conjunction with the block AI bots option. We found through testing on our own site that the block AI option is applied at a higher precedence. However, if a site is using the block definately automated setting, we cannot infer whether the site is also using the block AI bots setting. This is because the set of AI bots blocked is a strict subset of the set of "definately automated" user-agents. Thus, for some sites, it is impossible to infer whether the site is using both the block AI Bots features and have set the "Definately Automated" setting to "Block", or is just using the latter setting. However, if a site has "Definately Automated" set to "Allow" or "Managed Challenge", then we can accurately infer if the site has opted to block AI bots or not. 

% How do we infer each setting?
To test which setting (Block/Allow/Managed Challenge) a site is using for the "Definately Automated" rule, we visit the site with a user-agent that is a verified bot, but not an AI bot (e.g., GoogleBot), from the "wrong" IP address. If the site our request is met with the Cloudflare Block page, then the site is using the "Block" setting. If the site is met with the Cloudflare Challenge page, then the site is using the "Managed Challenge" setting. If the site is met with the site's content, then the site is using the "Allow" setting.

Then, we visit the site with a user-agent of an AI bot. If in the previous step we determined that the site has set Definately Automated to "Allow" or "Challenge", then if our AI bot request blocked, then this means that the site has enabled the block AI bots option. However, if in the previous step we detemined that the site has set Definately Automated to "Block", then we are unable to determine whether our request is being block by the AI bots option or the definately automated option, because as mentioned above, there is no user agent that is blocked by the AI bots option but not the Definately Automated option.

\paragraph{Results} In summary, we were able to determined the setting for \todo{XX}\% of sites using Cloudflare. We find that \todo{XX}\% of sites using Cloudflare have the "Block AI Bots" option enabled. There is a subset of sites that we were unable to determine the setting as they may have been using 3rd party blocking mechanisms, or have some custom, non-standard Cloudflare WAF configurations. We also find that the rate of sites soley blocking the fake GoogleBot is relatively high, at around 22\%. This may be because there was a lot of publicitly about blocking Googlebot imposters at some point.
\todo{put table of results in here}


% \subsection{Testing Major Hosting Services / CDNs} 
% The goal of this section is two-fold. First, we investigate the default bot-blocking behvaior of major hosting services / reverse proxies so that we can validate that our results in section\todo{XXX} are not biased by the default blocking behavior of these services. Second, we evaluate the difficulty in setting up blocking AI bots and discuss some of the challenges and limitations of these blocking mechanisms.

% First, we validate that the default blocking behavior of major hosting services / CDNs is not biasing our dataset.
% That is, our results reflect a concious attempt to block AI bots, rather than a CDN's default blocking behavior.
% We test the default blocking behavior of major hosting services and CDNs to see if they block AI bots by default. We created free and paid accounts at Cloudflare, \todo{Linode (Akamai), and AWS} and first tested a variety of common web automation tools and simulated crawls on a test website using different AI user-agent strings. Table \todo{xxx} shows the result of the experient. We find that by default, both the free and \todo{paid} Cloudflare setups do not block AI bots by default. \todo{Linode and AWS results}
\subsection{Results}
\todo{Need to add more detailed resutls}
We find that in practice, many websites block AI and crawler user-agents much more comprehensively than their rules in robots.txt. Table \ref{table:ai_bots_blocked} shows the percentage of AI bots that are disallowed in robots.txt versus the percentage that are blocked in practice for common AI bot user-agents.
Interestingly, \todo{XXX Percent} of websites do not have robots.txt or any rules in robots.txt yet they still block AI bots.
This suggests that many/some websites do not bother with updating their robots.txt file and instead rely on active blocking mechanisms to prevent unwanted bots and crawlers.

\begin{table}[ht]
\centering
\begin{tabular}{|l|c|c|}
\hline
% \textbf{Bot Name} & \textbf{\% disallowed \newline in robots.txt} & \textbf{\% blocked \newline in practice} \\ \hline
\textbf{Bot Name} & \makecell{\textbf{\% disallowed} \\ \textbf{in robots.txt}} & \makecell{\textbf{\% blocked} \\ \textbf{in practice}} \\ \hline
GPTBot            & 14.5                                  & 0.0                             \\ \hline
ChatGPT-User      & 12.6                                  & 0.0                             \\ \hline
Claude            & 0.0                                  & 0.0                             \\ \hline
Bing AI           & 0.0                                  & 0.0                             \\ \hline
Bard              & 0.0                                  & 0.0                             \\ \hline
Anthropic         & 0.0                                  & 0.0                             \\ \hline
Jasper            & 0.0                                  & 0.0                             \\ \hline
Perplexity AI     & 0.0                                  & 0.0                             \\ \hline
YouChat           & 0.0                                  & 0.0                             \\ \hline
Neeva AI          & 0.0                                  & 0.0                             \\ \hline
\end{tabular}
\caption{AI bot user-agents disallowed in robots.txt versus blocked in practice}
\label{tab:ai_bots_blocked}
\end{table}

\subsection{Content Management Systems}
\todo{We can consider moving this subsection to the robots.txt section, as it is related to agency over modifying robots.txt, rather than actual blocking behavaviors.}
Given that many users who post copyright-protected content in the internet are not technically inclined, many use web hosting platorms that provide a user-friendly interface for creating websites. 
In this section, we investigate the agency these web hosting provides provide for a user when configuring AI-blocking options. 

We investigated the top \todo{XXX} web hosting providers used by artists in our dataset. Table \todo{XXX} shows a breakdown of the proportion of artists that use each hosting provider. We then investigate 1. the default robots.txt file provided by the platform (if one is provided), and 2. the options the user has for modifying robots.txt (if provided by the site). Table \ref{tab:webhostingresults} summarizes these results.


\begin{table}
    \centering
    \begin{tabular}{|l|c|c|}
    \hline
    \textbf{CMS} & \textbf{Edit directly?} & \textbf{Options} \\ \hline
    Artstation & No & None \\ \hline
    Squarespace & No & Block AI, Block SE \\ \hline
    Weebly & No & Block SE \\ \hline
    Wix (Free) & No & None \\ \hline
    Wix (Paid) & Yes & Edit \\ \hline
    Godaddy & Yes & Upload \\ \hline
    Medium & No & None \\ \hline
    Substack & No & None \\ \hline
    Carbonmade & No & None \\ \hline
    Adobe Portfolio & No & Block SE \\ \hline
    \end{tabular}
    \caption{Overview of Content Management Systems (CMS) and Their Editing Capabilities \todo{add which AI bots they block in default robots.txt}}
    \label{tab:webhostingresults}
\end{table}
    
Next, for the artists that use Squarespace, we check what percent of users have enabled the "Block AI Bots" option. We find that only 17\% of artists have enabled this option. This suggests that many artists, despite generally caring about AI scraping, are either unaware of this option or do not care enough to enable it.

\subsection{Discussion of Challenges with Bot Mitigation Tools}
% \todo{This is more related to the cloudflare and cloudfront analysis, rather than the artist sites analysis which is more targeted towards robots.txt}
In summary, we find several challenges with the current state of bot mitigation tools and robots.txt enforcement:
\begin{itemize}
    \item \textbf{Lack of Transparency:} The list of AI bots blocked is not publically availible, making it difficult for website operators to know what is being blocked.
    \item \textbf{Lack of agency and fine-grained control:} The Cloudflare "Block AI Bots" option is a binary switch, and does not allow for fine-grained control over which bots are blocked.
    \item \textbf{Effectiveness of blocking mechanisms:} The Cloudflare "Block AI Bots" option is easily evaded trival changes in the user-agent string.
    \item \textbf{Incomplete list of bots to block:} The Cloudfront AI category only blocks GPTBot and GPTUser, which is not comprehensive. Cloudflare blocks more AI user-agents, but the list is far from complete.
    \item \textbf{Disconnect between robots.txt and actual blocking behavior:} We find that many sites have conflicts between their stated intent in robots.txt versus their actual blocking behavior. 
\end{itemize}

\para{Existing Tools for Robots.txt enforcement:} There are limited tools, one is Dark Visitors, which provides a Wordpress Extension that enforces robots.txt. We leave it to future work to develop a tool that can universally sync robots.txt with actual blocking behavior.

% Lack of Transparency

% Lack of agency and fine-grained control

% Effectiveness of blocking mechanisms

% Incomplete list of bots to block

% Disconnect between robots.txt and actual blocking behavior

% We could also mention that dark visitors is a tool that exists that attempts to enforce robots.txt rules. 



==> method.tex <==

\section{Understanding Creators' Anti-crawling Practices and Preferences}

\para{Ongoing Struggle against AI scraping. } \ol{summarize a bit more concrete example of creator's struggle against AI}

\para{Key Questions. }

\begin{packed_itemize}

\item do they host their websites

\item do they want to block

\item do they use things like robots.txt 

\item what about the largest content websites. what do they think about AI scraping. 

\end{packed_itemize}





\begin{table}[t]
  \centering
  \resizebox{0.5\textwidth}{!}{
  \centering
\begin{tabular}{lcc}
\hline
	\textbf{Website Type} & \textbf{\# of Sites} & \textbf{Sources} \\ \hline
Individual Artist & \fixme{1,000} & Artists Unions \\
Large Content Holder & \fixme{1,000} & Tranco + HEAD2K \\
Top 100K  & \fixme{50,000} & Tranco \\ \hline
	\end{tabular}
  }
  \caption{Dataset info}
  \label{tab:dataset}
\end{table}











